Hypervelocity Stars: From the Galactic Center to the Halo

Hypervelocity stars (HVS) traverse the Galaxy from the central black hole to the outer halo. We show that the Galactic potential within 200 pc acts as a high pass filter preventing low velocity HVS from reaching the halo. To trace the orbits of HVS throughout the Galaxy, we construct two forms of the potential which reasonably represent the observations in the range 5--100,000 pc, a simple spherically symmetric model and a bulge-disk-halo model. We use the Hills mechanism (disruption of binaries by the tidal field of the central black hole) to inject HVS into the Galaxy and compute the observable spatial and velocity distributions of HVS with masses in the range 0.6--4 Msun. These distributions reflect the mass function in the Galactic Center, properties of binaries in the Galactic Center, and aspects of stellar evolution and the injection mechanism. For 0.6--4 Msun main sequence stars, the fraction of unbound HVS and the asymmetry of the velocity distribution for their bound counterparts increases with stellar mass. The density profiles for unbound HVS decline with distance from the Galactic Center approximately as r^{-2} (but are steeper for the most massive stars which evolve off the main sequence during their travel time from the Galactic Center); the density profiles for the bound ejecta decline with distance approximately as r^{-3}. In a survey with a limiting visual magnitude V of 23, the detectability of HVS (unbound or bound) increases with stellar mass.

==> README-REVISION <==
20 February 2008


Prof. W. Butler Burton
Associate Editor-in-Chief, The Astrophysical Journal
Professor Emeritus, Leiden University  
National Radio Astronomy Observatory


Dear Prof. Burton:

I have submitted a revised version of the paper, 
``Hypervelocity Stars: From the Galactic Center to 
the Halo,'' by S. J. Kenyon, B. C.  Bromley, 
M. J. Geller, and W. R. Brown.

We thank the referee for their prompt review of our
manuscript.  We are pleased the comments are minor.
In addition to these comments, several colleagues
suggested some revisions to the text. Below, we 
append the referee's comments, our responses to the 
referee (indicated by ***** following the reviewer's 
comment), and our changes in response to comments 
from colleagues (indicated by ***** followed by 
(a) through (g) at the end of this letter).

We hope the paper is now acceptable for publication.

Sincerely,
Scott Kenyon
(e-mail: skenyon@cfa.harvard.edu)



----------------------------------------------------------------
This is a paper concerning the distribution of the so-called
hypervelocity stars within the Galaxy.

This is an interesting piece of work, which is clear and well 
set out.

In my opinion, the paper is acceptable for publication once 
the following points have been addressed by the authors:


Equation (3) in section 2.1 could be written more clearly. 
It would be easier to understand if written in the form:

f_R = a1*D + a2*D*D + ...

***** We disagree with the referee on this point. The form of
this equation is identical to that in Bromley et al.  (2006) 
and is appropriate for a C or a FORTRAN program. Changing the
form in this paper might give readers the false impression that
the coefficients have changed. We prefer to avoid any chance 
of confusion and therefore leave the equation unchanged.

At the end of section 2.1, the authors should include
a more quantitative discussion of whether the primary
or the secondary of the binary is ejected. Perhaps
a plot of f_primary vs q?

***** This comment is confusing. In the next to the last 
paragraph of sec 2.1, we state: 'ejections of the primary and 
secondary star are equally likely'.  In the following paragraph, 
we state, 'Our simulations suggest that the binary mass ratio 
affects the ejection probability only when the mass ratio is 
extreme (q > 10). There is then a consistent preference for 
ejection of the secondary.' 

***** In Bromley et al (2006), we described the fate of the 
primary and secondary in more detail, coming to the same 
conclusion. ``for the types of binary orbits and mass ranges 
we consider, the primary and secondary have an approximately
equal chance of ejection.''

***** A plot of f_primary vs q might be interesting for q > 10.
However, the plot is not interesting for cases considered in 
this paper (q < 7), where f_primary ~= f_secondary ~= 0.5. 

***** To refer readers to the discussion in Bromley et al (2006),
we added a reference to the end of a sentence (p. 8): `There is 
then a consistent preference for ejection of the secondary 
\citep[for additional details, see][]{bkg06}.'  This addition
informs the reader that we have a broader discussion in our first
paper.


Collisions can play an important role. A recent paper by Ginsburg 
and Loeb (2007) discusses the collision rate. In the paper 
submitted here, the authors should cite the Ginsburg paper and 
discuss how frequent collisions between the stars within the binary 
will be as they pass close to the supermassive black hole. I suspect 
that this rate will not be negligible, especially for the very tight 
binaries (ie close to amin from Table 1). 

***** We chose a_min to minimize the chance of a collision. Based 
on Ginsburg and Loeb (2006), we estimated a collision probability 
of roughly 10% for the minimum binary separations used in Bromley 
et al (2006). This probability is comparable to the collision 
probability derived from Table 1 in Ginsburg and Loeb (2007). For 
a 3 + 3 Msun binary, Ginsburg and Loeb (2007) quote p = 11% for 
a = 0.1 AU and p = 6% for a = 0.15 AU. For our a_min = 0.115 AU, 
we estimate p = 9.5%. Compared to the other uncertainties in the
problem - such as the exact forms of the Galactic potential and
initial mass function - this probability is small.

***** To make it clear that we have considered the possibility of 
collisions during the encounter, we modified the text preceeding 
equation (1): `To minimize the probability of a collision during 
the encounter (<= 10\%), we set $a_{min}$ = 2 $R_{ms,1} / r_L$ 
\citep[see also Table 1 of][]{gin07}, where $R_{ms,1}$ is the 
radius of the primary star and ...' 

***** This change adds the reference requested by the referee and 
allows the interested reader to compare our a_min with Table 1 of 
Ginsburg and Loeb. In the original text and in Bromley et al. (2006), 
we note that collisions and possible coalescence might change our 
ejection probabilities by 10%. We left this text unchanged, but we 
added a reference to Ginsburg and Loeb 2007 to point the reader to
this more recent study.


There are two other recent papers which should be cited by the 
authors.

Svensson et al, 2008, MNRAS, 383, L15 -- which considers the 
trajectories of the observed hypervelocity stars and discusses the 
origin of the one system seen moving towards the galactic center.

***** We added a citation to this paper in the introduction
(p. 4, paragraph 2).

O'Leary and Loeb, 2008, 383, 86 -- which is an interesting paper 
discussing an alternative idea where the stars are scattered by 
a cluster of stellar-mass black holes.

The current reference in the reference list for O'leary and Loeb 
is incomplete.

***** We cited this paper in the introduction and thank the 
referee for pointing out the updated reference.


***** Based on comments from other colleagues and our own
re-reading of the manuscript, we made the following additional 
changes.

***** (a) corrected various typos and updated references 

***** (b) added minus signs to equation (8) and equation (9)

***** (c) to clarify our model potential for the Milky Way,
we added a footnote stating that we reduce the scale length
in the Klypin et al model from 5 kpc to 4 kpc. In Tables 2-3, 
we correct an error in the disk scale length and the disk
mass for this model.

***** (d) We added a reference to a new paper by Widrow et al
on mass models of galaxies, including the Wilky Way.

***** (e) We added a paragraph to provide a better context for
our comparison of Galaxy potentials in Fig. 1 (p. 11):

To illustrate how the acceleration varies among different potentials,
Figure \ref{fig:gaxmodacc} compares $|a|$ for our simple spherical
potential with the three component model adopted here and a three
component model developed to analyze HVS trajectories in a triaxial
Milky Way halo \citep{gne05}. Most other Galaxy potentials have
acceleration profiles similar to the \citet{gne05} potential
\citep[e.g.][]{deh98,klyp02,bat05,deh06,yu07}. Because the 
\citet{wid05} potential overestimates the mass in the \GC, this
model overestimates $|a|$ in the \GC.

***** (f) We added a footnote to clarify that our potential is
constant in time (p. 13):

\footnote{We assume a constant Galactic potential.  Because the 
Galaxy probably gains mass with time \citep[e.g.][]{bul05}, our 
estimates for the bound population of older, less massive stars 
are more uncertain than estimates for more massive stars.}

***** (g) We added a footnote to clarify our choices for the
binary frequency as a function of stellar mass (p. 22, first 
paragraph):

\footnote{Other physical processes -- including binary evaporation
near the MBH \citep{per07b} and interactions between binaries and
molecular clouds \citep{per07} -- can lower the relative abundance
of solar-type stars among HVS. To maximize the predicted density of
low mass stars among HVS, we ignore these processes in our estimate
of $x_2$.}

***** (h) To compare our results for the bulge potential with Genzel's 
measurements of the central few pc of the Galactic Center, we added 
two sentences in the middle of p. 10:

This model for the bulge underestimates the stellar mass within a few
pc of the \GC\ \citep{gen03}. Because mass in the central 10--100 pc
has the largest impact on HVS trajectories, this underestimate has
little impact on our results.

